StreamTinyNet: video streaming analysis with spatial-temporal TinyML

Tiny Machine Learning (TinyML) is a branch of Machine Learning (ML) that constitutes a bridge between the ML world and the embedded system ecosystem (i.e., Internet of Things devices, embedded devices, and edge computing units), enabling the execution of ML algorithms on devices constrained in terms of memory, computational capabilities, and power consumption. Video Streaming Analysis (VSA), one of the most interesting tasks of TinyML, consists in scanning a sequence of frames in a streaming manner, with the goal of identifying interesting patterns. Given the strict constraints of these tiny devices, all the current solutions rely on performing a frame-by-frame analysis, hence not exploiting the temporal component in the stream of data. In this paper, we present StreamTinyNet, the first TinyML architecture to perform multiple-frame VSA, enabling a variety of use cases that requires spatial-temporal analysis that were previously impossible to be carried out at a TinyML level. Experimental results on public-available datasets show the effectiveness and efficiency of the proposed solution. Finally, StreamTinyNet has been ported and tested on the Arduino Nicla Vision, showing the feasibility of what proposed.

==> Tab_comparison.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c c c |}
    \hline
     & \textbf{Mean} & \textbf{Variance} \\
    \hline \hline
    {Accuracy} & 0.46 &  0.0012 \\
    {Precision} & 0.91 & 0.0005 \\
    {Recall}  & 0.46 &  0.0012 \\
    {F1 score} & 0.57 & 0.0015 \\
    {PCE} & 0.56 & 0.0002 \\
    \hline
    \end{tabular}
    \caption{Results of the proposed architecture with of $T = 16$}
    \label{table:goolfDB_results_t15}
\end{table}

==> Tab_complexity_1.tex <==
\begin{table*}
    
    \centering 
    \begin{tabular}{|c|c|c|c|}
    \hline
   
    &\textbf{Memory Footprint} & \textbf{ Computational Load} & \textbf{Output Dim.}  \\
    \hline \hline
    $I$ & $M_{in}\times N_{in}\times C_{in}$ & - & $M_{in}\times N_{in}\times C_{in}$\\
    \hline \hline
    CONV-$1$ & $ r^{(1)^2} \times C_{in} \times n^{(1)}+ M_{in}\times N_{in}\times n^{(1)}$ & $ r^{(1)^2}\times C_{in}\times n^{(1)}\times M_{in}\times N_{in}$ & $M_{in}\times N_{in}\times n^{(1)}$\\
    POOL-$1$ & $ 0 + \frac{M_{in}}{2}\times \frac{N_{in}}{2}\times n^{(1)}$ & $2\times 2\times M_{in}\times N_{in} \times n^{(1)}$ & $\frac{M_{in}}{2}\times \frac{N_{in}}{2}\times n^{(1)}$\\
    \hline \hline
    \vdots &\vdots &\vdots & \vdots\\
    \hline \hline
    CONV-$l$ & $ r^{(l)^2} \times n^{(l-1)} \times n^{(l)} + \frac{M_{in}}{2^{l-1}}\times \frac{N_{in}}{2^{l-1}}\times n^{(l)}$ & $ r^{(l)^2}\times n^{(l-1)}\times n^{(l)}\times \frac{M_{in}}{2^{l-1}}\times \frac{N_{in}}{2^{l-1}}$ & $\frac{M_{in}}{2^{l-1}}\times \frac{N_{in}}{2^{l-1}}\times n^{(l)}$\\
    POOL-$l$ & $ 0 + \frac{M_{in}}{2^{l-1}}\times \frac{N_{in}}{2^{l-1}}\times n^{(l)}$ & $2\times 2\times\frac{M_{in}}{2^{l-1}}\times \frac{N_{in}}{2^{l-1}} \times n^{(l)}$ & $\frac{M_{in}}{2^{l-2}}\times \frac{N_{in}}{2^{l-2}}\times n^{(l)}$\\
    \hline \hline
    $O$ & - & - & $M_{out}\times N_{out}\times C_{out}$\\
    \hline
    \end{tabular}
    %\\[10pt]
     \caption{The memory footprint and computational load of the sublayers of $g$ (see Figure \ref{fig:feature_extractor})}
    
   
\end{table*}

\begin{table*}
    
    \centering 
    \begin{tabular}{|c|c|c|c|}
    \hline
    &\textbf{Memory Footprint} & \textbf{ Computational Load} & \textbf{Output Dim.}  \\
    \hline \hline
    $O^T$ & $M_{out}\times N_{out}\times C_{out} \times T$ & - & $M_{out}\times N_{out}\times C_{out} \times T$\\
    \hline \hline
    CONV($1\times 1$) & $C_{out}\times (T + M_{out}\times N_{out})$ & $ C_{out}\times T \times M_{out}\times N_{out}$ & $M_{out}\times N_{out}\times C_{out}$\\
    \hline \hline    
    FLATTEN & - & - & $x = M_{out}\times N_{out}\times C_{out}$\\
    \hline \hline
    DENSE-$1$ & $(x\times d^{(1)}) + (d^{(1)})$ & $x\times d^{(1)}$ & $d^{(1)}$\\
     \vdots &\vdots &\vdots & \vdots\\
    DENSE-$b$ & $( d^{(b-1)} \times d^{(b)}) + (d^{(b)})$ & $d^{(b-1)}\times d^{(b)}$ & $d^{(b)}$\\

    
    SOFTMAX & $(d^{(b)}\times k) + (k)$ & $d^{(b)}\times k$ & $k$\\
    \hline
    \end{tabular}
    %\\[10pt]
     \caption{The memory footprint and computational load of the sublayers of $h$ (see Figure \ref{fig:abstract_network_h})}
    \label{table:complexity_h}
   
\end{table*}

==> Tab_device_specs.tex <==
\begin{table*}
    \caption{Raspberry Pi 4 and Arduino Nicla Vision specifications}
    \label{table:porting_spec}
    \centering
    \begin{tabular}{|p{8em} |p{15em}|p{15em}|}
    \hline
     & \textbf{Raspberry Pi 4} & \textbf{Arduino Nicla Vision}  \\
    \hline \hline
    \textbf{Processing Power} & Broadcom BCM2711, Quad core Cortex-A72 (ARM v8) & STM32H747AII6 Dual Arm Cortex M7/M4 IC  \\

    \hline \hline
    \textbf{Memory} & 8GB LPDDR4 RAM & 2MB Flash / 1MB RAM  \\

    \hline \hline
    \textbf{Camera Sensor} & External camera through its dedicated camera interfaces & Integrated 2 MP Color Camera  \\

    % \hline \hline
    % \textbf{AVG Power Consumption} & - & $105 mA$ during image capturing $374\mu A$ in deep sleep mode  \\

    \hline \hline
    \textbf{Dimensions} &$ 85.6mm \times 56.5mm \times 17mm$ & $22.86mm \times 22.86mm \times 10mm$  \\    
    \hline
    \end{tabular}
\end{table*}

==> Tab_different_T2.tex <==
\begin{table*}
   \centering 
    \begin{tabular}{|c| c c c| c c c c c c|}
    \hline
    & \multicolumn{3}{c|}{\textbf{SwingNet-160}} & \multicolumn{6}{c|}{\textbf{\networkNameNoSpace}}\\
    
    \hline\hline
    T &PCE&c ($10^9$ FLOPs)& $m_w$ &PCE& c ($10^9$ FLOPs) & $m_w$ & $m_a$* & $m_f$ & $m$\\
    \hline\hline
    4&0.63& 0.68& $5,380,000$ &0.48&0.007992& 115,920 & 187,200 & 6,400 & 309,520\\
    8&0.66&1.35& $5,380,000$ &0.51& 0,008005& 116,176 & 193,600 & 12,800 & 322,576\\
    16&0.71&2.70 & $5,380,000$ &0.55& 0,008031& 116,688 & 206,400 & 25,600 & 348,688\\
    32&0.74&5.41& $5,380,000$ & - & 0,008082 & 117,712 & 232,000 & 51,200 & 400,912\\
    64&0.76&10.92& $5,380,000$& - & 0,008184 & 119,760 & 283,200 & 102,400 & 505,360\\

    \hline
    \end{tabular}
     \caption{Evaluation results from different values of T. *Optimization is on.}
    \label{table:goolfDB_increasing_T-dataset}
    
\end{table*}

==> Tab_metrics.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c c c c|}
    \hline
    %\multicolumn{5}{|c|}{\textbf{\networkNameNoSpace}} \\ p{1.4cm} p{1.4cm} p{1.4cm} p{1.4cm} p{1.4cm}
    \textbf{Acc.} & \textbf{Pre.}& \textbf{F1} & \textbf{PCE} \\
    \hline \hline
    $0.46 \pm 0.03$ & $0.91 \pm 0.02$ & $0.57 \pm 0.04$ & $0.56 \pm 0.01$ \\
    %$0.46 \pm 0.034$ & $0.91 \pm 0.022$  &  $0.57 \pm 0.038$ & $0.56 \pm 0.014$ \\
    \hline
    \end{tabular}
    \caption{Detailed results of the proposed \networkName($T = 16$) with confidence intervals.}
    \label{table:goolfDB_results_best_solution}
\end{table}

==> param_golf.tex <==
\begin{table}
    \centering 
    \begin{tabular}{|c c c c c | c | c c c|}
    \hline
    $n^{(1)}$ & $n^{(2)}$ & $n^{(3)}$ & $n^{(4)}$ & $n^{(5)}$ & $r^{(-)}$ & $d^{(1)}$ & $d^{(2)}$ & $k$ \\
     \hline\hline
     $4$ &$8$ &$16$ &$32$ &$64$ & 2 & $64$ & $32$ & 9\\
    \hline
    \end{tabular}
    %\\[10pt]
    \caption{Overview of the parameters of \networkName used for the GolfDB}
     \label{table:parameter_summary-golf}
\end{table}

\begin{table}
    \centering 
    \begin{tabular}{|c|c|}
    \hline
     \textbf{Parameter} & \textbf{description}  \\
     \hline\hline
      $T$ & 1,4,8,16\\
    \hline \hline
         $l$ & $5$\\
         \hline
         $n^{(1)}$ & $4$ \\
         $n^{(2)}$ &$8$\\
         $n^{(3)}$ &$16$\\
         $n^{(4)}$ &$32$\\
         $n^{(5)}$ &$64$\\
         \hline
         $r^{(-)}$ & 2\\
    \hline\hline
         $b$ & 2\\
         $d^{(1)}$ & $64$\\
         $d^{(2)}$& $32$\\
         $k$ & 9\\
    \hline
    \end{tabular}
    %\\[10pt]
    \caption{Overview of the parameters of \networkName used for the GolfDB}
     \label{table:parameter_summary-golf}
\end{table}

\begin{table}
    \centering 
    \begin{tabular}{|c|c|}
    \hline
      \textbf{Parameter} & \textbf{description}  \\
     \hline\hline
      $T$ & 10 \\
    \hline \hline
      $l$ & $4$\\
      \hline\hline
         $n^{(1)}$ & $4$\\
         $n^{(2)}$ & $8$\\
         $n^{(3)}$ & $16$\\
         $n^{(4)}$ & $32$\\
         \hline\hline
         $r^{(-)}$ & 2\\
    \hline\hline
        $b$ & 1\\
        $d^{(1)}$ & $16$\\
         $k$ & 3\\
    \hline
    \end{tabular}  
     \caption{Overview of the parameters of the \networkName used for the JesterDB}
    \label{table:parameter_summary-jester}
\end{table}
